UniMC: Taming Diffusion Transformer for Unified Keypoint-Guided Multi-Class Image Generation

Although significant advancements have been achieved in the progress of keypoint-guided Text-to-Image diffusion models, existing mainstream keypoint-guided models encounter challenges in controlling the generation of more general non-rigid objects beyond humans (e.g., animals). Moreover, it is difficult to generate multiple overlapping humans and animals based on keypoint controls solely. These challenges arise from two main aspects: the inherent limitations of existing controllable methods and the lack of suitable datasets. First, we design a DiT-based framework, named UniMC, to explore unifying controllable multi-class image generation. UniMC integrates instance- and keypoint-level conditions into compact tokens, incorporating attributes such as class, bounding box, and keypoint coordinates. This approach overcomes the limitations of previous methods that struggled to distinguish instances and classes due to their reliance on skeleton images as conditions. Second, we propose HAIG-2.9M, a large-scale, high-quality, and diverse dataset designed for keypoint-guided human and animal image generation. HAIG-2.9M includes 786K images with 2.9M instances. This dataset features extensive annotations such as keypoints, bounding boxes, and fine-grained captions for both humans and animals, along with rigorous manual inspection to ensure annotation accuracy. Extensive experiments demonstrate the high quality of HAIG-2.9M and the effectiveness of UniMC, particularly in heavy occlusions and multi-class scenarios.

==> sec/00_teaser.tex <==
% \begin{figure}[http]
% \begin{figure*}[t]
\begin{figure*}[htbp]
  \centering
  % \vspace{-12pt}
  % \includegraphics[width=0.98\linewidth]{figs/teaser.pdf}

    \begin{tabular}{c}
    \includegraphics[width=0.95\linewidth]{figs/teaser.pdf} \\
    \end{tabular}


  \caption{\textbf{Top:} We establish \datasetname, a large-scale, high-quality, and highly diverse dataset with joint keypoint-level, instance-level, and densely semantic annotations for non-rigid humans and animals.
  \textbf{Bottom:} Based on \datasetname, we design \modelname, a controllable DiT-based framework for keypoint position-guided image generation, especially for heavy occlusion and multi-class scenarios. 
  }


  
  \label{fig:teaser}
  \vspace{-0.6cm}
% \end{wrapfigure}
\end{figure*}




==> section/imgs/qualitative.tex <==
\begin{figure*}[h!]
  \centering
  \includegraphics[width=0.96\linewidth]{figs/qualitative.pdf}\vspace{-3pt}
  \caption{
  \textbf{Qualitative Comparisons.} 
  We provide all methods with required condition formats. 
  \textbf{From left to right:}
  % 
  \textbf{(a)}: Input condition, \textbf{(b)}: \modelname~trained on \datasetname, \textbf{(c)}: \modelname~trained on COCO, \textbf{(d)}: \modelname~trained on APT36K, \textbf{(e)}: \modelname~trained on COCO+APT36K, \textbf{(f)}: ControlNet, \textbf{(g)}: GLIGEN.
  }
  \label{fig:qualitative}
  % \vspace{-16pt}
\end{figure*}


==> section/tabs/ablation_controller.tex <==
\begin{table*}[http!]
\caption{\textbf{Quantitative Results on Different Methods}. We compare our model with \modelalpha~\citep{chen2024pixartalpha} and keypoint-guided methods~\citep{zhang2023adding,li2023gligen}. For \modelalpha and \modelname, we first generate $1024\times1024$ results, then resize back to $512\times512$.
}
\footnotesize
\setlength{\tabcolsep}{4.4pt}
\centering
\small
\begin{tabular}{ccccccccc}
\toprule
& \multicolumn{2}{c}{Image Quality} & \multicolumn{1}{c}{Alignment} &  \multicolumn{2}{c}{Class Accuracy (\%)} &  \multicolumn{2}{c}{Pose Accuracy (AP)} \\
\cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8}
Methods & FID $\downarrow$ & $\text{KID}_{\text{\tiny $\times 1\mathrm{k}$}} \downarrow$ & CLIP $\uparrow$ & Human $\uparrow$ & Animal $\uparrow$ & Human $\uparrow$ & Animal $\uparrow$\\
\midrule
\modelalpha & \textbf{23.50} & \textbf{7.52} & 32.17 & - & - & - & - \\
ControlNet & 26.72 & 8.90 & \underline{32.20} & \underline{90.67} & \underline{52.03} & \underline{29.01} & \underline{20.29} \\
GLIGEN & 31.01 & 11.15 & 31.44 & 82.06 & 9.90 & 26.58 & 3.96 \\
\midrule 
\modelname~(ours) & \underline{23.63} & \underline{7.57} & \textbf{32.28} \textcolor{red}{\scriptsize $_{0.2\%\uparrow}$} & \textbf{93.55} \textcolor{red}{\scriptsize $_{3.2\%\uparrow}$} & \textbf{91.71} \textcolor{red}{\scriptsize $_{76.3\%\uparrow}$} & \textbf{30.01} \textcolor{red}{\scriptsize $_{3.4\%\uparrow}$} & \textbf{28.38} \textcolor{red}{\scriptsize $_{39.9\%\uparrow}$} \\
\bottomrule
\end{tabular}
\label{tab:res}
\vspace{-12pt}
\end{table*}


==> section/tabs/dataset_comparison.tex <==
\begin{table*}[http!]
% \begin{table*}[h]
\vspace{-9pt}
\caption{\textbf{Quantitative Results on Different Training Datasets.} 
We bold the \textbf{best} and underline the \underline{second} results. Our improvements over the second method are shown in \textcolor{red}{red}.}
\footnotesize
\setlength{\tabcolsep}{1.5pt}
\centering
\small
\begin{tabular}{ccccccccc}
\toprule
& \multicolumn{2}{c}{Image Quality} & \multicolumn{1}{c}{Alignment} &  \multicolumn{2}{c}{Class Accuracy (\%)} &  \multicolumn{2}{c}{Pose Accuracy (AP)} \\
\cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8}
Dataset & FID $\downarrow$ & $\text{KID}_{\text{\tiny $\times 1\mathrm{k}$}} \downarrow$ & CLIP $\uparrow$ & Human $\uparrow$ & Animal $\uparrow$ & Human $\uparrow$ & Animal $\uparrow$\\
\midrule
COCO & 45.08 & 18.75 & 28.07 & 45.33 & 4.63 & 19.25 & 1.52 \\
APT36K & 43.72 & 18.20 & 29.00 & 21.96 & 48.95 & 5.64 & 19.52 \\
COCO+APT36K & \underline{33.79} & \underline{13.55} & \underline{32.10} & \underline{67.97} & \underline{67.83} & \underline{25.69} & \underline{21.07} \\
\midrule 
\datasetname~(ours) & \textbf{23.63} \textcolor{red}{\scriptsize $_{30.1\%\downarrow}$} & \textbf{7.57} \textcolor{red}{\scriptsize $_{44.1\%\downarrow}$} & \textbf{32.28} \textcolor{red}{\scriptsize $_{0.6\%\uparrow}$} & \textbf{93.55} \textcolor{red}{\scriptsize $_{37.6\%\uparrow}$} & \textbf{91.71} \textcolor{red}{\scriptsize $_{35.2\%\uparrow}$} & \textbf{30.01} \textcolor{red}{\scriptsize $_{16.8\%\uparrow}$} & \textbf{28.38} \textcolor{red}{\scriptsize $_{34.7\%\uparrow}$} \\
\bottomrule
\end{tabular}
\label{tab:res_dataset}
% \vspace{-15pt}
\end{table*}


==> section/tabs/method_comparison.tex <==
\begin{table*}[http!]
\caption{\textbf{Quantitative Results on Different Methods}. We compare our model with \modelalpha~\citep{chen2024pixartalpha} and keypoint-guided methods~\citep{zhang2023adding,li2023gligen}. For \modelalpha and \modelname, we first generate $1024\times1024$ results, then resize back to $512\times512$.
}
\footnotesize
\setlength{\tabcolsep}{4.4pt}
\centering
\small
\begin{tabular}{ccccccccc}
\toprule
& \multicolumn{2}{c}{Image Quality} & \multicolumn{1}{c}{Alignment} &  \multicolumn{2}{c}{Class Accuracy (\%)} &  \multicolumn{2}{c}{Pose Accuracy (AP)} \\
\cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8}
Methods & FID $\downarrow$ & $\text{KID}_{\text{\tiny $\times 1\mathrm{k}$}} \downarrow$ & CLIP $\uparrow$ & Human $\uparrow$ & Animal $\uparrow$ & Human $\uparrow$ & Animal $\uparrow$\\
\midrule
\modelalpha & \textbf{23.50} & \textbf{7.52} & 32.17 & - & - & - & - \\
ControlNet & 26.72 & 8.90 & \underline{32.20} & \underline{90.67} & \underline{52.03} & \underline{29.01} & \underline{20.29} \\
GLIGEN & 31.01 & 11.15 & 31.44 & 82.06 & 9.90 & 26.58 & 3.96 \\
\midrule 
\modelname~(ours) & \underline{23.63} & \underline{7.57} & \textbf{32.28} \textcolor{red}{\scriptsize $_{0.2\%\uparrow}$} & \textbf{93.55} \textcolor{red}{\scriptsize $_{3.2\%\uparrow}$} & \textbf{91.71} \textcolor{red}{\scriptsize $_{76.3\%\uparrow}$} & \textbf{30.01} \textcolor{red}{\scriptsize $_{3.4\%\uparrow}$} & \textbf{28.38} \textcolor{red}{\scriptsize $_{39.9\%\uparrow}$} \\
\bottomrule
\end{tabular}
\label{tab:res}
\vspace{-2pt}
\end{table*}

